HIDRA: Head Initialization across Dynamic targets for Robust Architectures

The performance of gradient-based optimization strategies depends heavily on the initial weights of the parametric model. Recent works show that there exist weight initializations from which optimization procedures can find the task-specific parameters faster than from uniformly random initializations and that such a weight initialization can be learned by optimizing a specific model architecture across similar tasks via MAML (Model-Agnostic Meta-Learning). Current methods are limited to populations of classification tasks that share the same number of classes due to the static model architectures used during meta-learning. In this paper, we present HIDRA, a meta-learning approach that enables training and evaluating across tasks with any number of target variables. We show that Model-Agnostic Meta-Learning trains a distribution for all the neurons in the output layer and a specific weight initialization for the ones in the hidden layers. HIDRA explores this by learning one master neuron, which is used to initialize any number of output neurons for a new task. Extensive experiments on the Miniimagenet and Omniglot data sets demonstrate that HIDRA improves over standard approaches while generalizing to tasks with any number of target variables. Moreover, our approach is shown to robustify low-capacity models in learning across complex tasks with a high number of classes for which regular MAML fails to learn any feasible initialization.

==> chapters/z-motivation.tex <==
\section{Motivation} \label{sec:motv}

Model Agnostic Meta-Learning methods such as \maml{} and \reptile{} \cite{finn2017model, reptile2018} aim to find the best initialization for the parameters $\theta$ of some model $f$ by training on a set of similar few-shot learning tasks $\D_\train$, thus allowing faster convergence for unseen tasks from the same knowledge domain.

These methods, however, don't work outside of the box for tasks which have different input and output sizes. To overcome this issue, some works such as \cham{} \cite{} allowed these methods to be able to project different input schema to a fixed shape for vector data, since, unlike images, we cannot re-scale these vectors in an intuitive way.

Ideally it would be of great benefit if \maml{} was able to have a flexible output layer, that could be trained with different output schema and be applied for any other output shape while keeping it scalable for any size.

==> plots/plotplots/plotComparisom.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{plots/Testfig}
\caption{Placeholder figure1} \label{plcaholder2}
\end{figure}
